InferCept: Efficient Intercept Support for Augmented Large Language Model Inference

Large language models are increasingly integrated with external environments, tools, and agents like ChatGPT plugins to extend their capability beyond language-centric tasks. However, today's LLM inference systems are designed for standalone LLMs. They treat each external interaction as the end of LLM generation and form a new request when the interaction finishes, causing unnecessary recomputation of already computed contexts, which accounts for 37-40% of total model forwarding time. This paper presents InferCept, the first LLM inference framework targeting augmented LLMs and supporting the efficient interception of LLM generation. InferCept minimizes the GPU resource waste caused by LLM interceptions and dedicates saved memory for serving more requests. InferCept improves the overall serving throughput by 1.6x-2x and completes 2x more requests per second compared to the state-of-the-art LLM inference systems.

==> Makefile <==
ifeq ($(OS),Windows_NT)
$(warning Windows NT detected "$(USER)")
DVI = yap
DVIBIN = yap
DISTILL = "$(HOME)"/bin/acrodist.exe
MY_DATE := $(strip $(shell date +"%F_%H_%M_%S"))
PREFIX=c:\\cygwin\\home\\$(USER)\\grants\\2007-cpa-arsenal\\
ACROREAD = "$(HOME)"/bin/acroread.exe
ALL = show_nt
else # mac
ALL =  pdf
endif

all: $(ALL)

PDF_TARGETS =main.pdf #zhang-bio.pdf facilities.pdf budget.pdf summary.pdf data-management.pdf zhang-collab.pdf

TEX_STUFF=$(wildcard *.tex) $(wildcard *.sty) $(wildcard *.cls) $(wildcard Figures/*.pdf) $(wildcard Graphs/*.pdf)

.PRECIOUS: .bbl .aux 

pdf: $(PDF_TARGETS)

# pdf: graphs
# 	rm -rf cpa.pdf
# 	pdflatex cpa
# 	bibtex cpa || true
# 	for i in bu?.aux; do bibtex $${i##.aux}; done
# 	pdflatex cpa
# 	pdflatex cpa

GRAPHS=

graphs: $(GRAPHS)

Graphs/%.pdf: Graphs/%.gnuplot.in
	cd Graphs; gnuplot < $*.gnuplot.in

%.aux : %.tex $(TEX_STUFF) 
	pdflatex $* 

%.bbl : %.aux 
	bibtex $* || true

%.pdf : %.bbl $(GRAPHS) $(FIGURES)
	pdflatex $*
	pdflatex $*
	pdflatex $*

test_build:
	rm -rf _test_build
	mkdir _test_build
	(cd _test_build; \
	 cvs checkout $$(cat ../CVS/Repository);\
	 cd $$(cat ../CVS/Repository);\
	 make;\
	)	

splitfiles:  main.pdf
	cp main.pdf proposal.pdf
	pdflatex proposaldesc.tex
#	pdflatex proposalsummary.tex
	pdflatex proposalbio.tex
#	pdflatex proposalbiotaylor.tex
	pdflatex proposalrelated.tex
#	pdflatex proposalequipment.tex
#	pdflatex proposalmanagement.tex

#
# copies file to prevent write-after-read problems
# uses date as suffix.
#

zhang-bio.pdf :  zhang-bio.tex $(TEX_STUFF)
	rm -rf zhang-bio.pdf
	pdflatex zhang-bio
	bibtex zhang-bio || true
	for i in bu?.aux; do bibtex $${i##.aux}; done
	pdflatex zhang-bio
	pdflatex zhang-bio

zhang-collab.pdf :  zhang-collab.tex $(TEX_STUFF)
	rm -rf zhang-collab.pdf
	pdflatex zhang-collab
	bibtex zhang-collab || true
	for i in bu?.aux; do bibtex $${i##.aux}; done
	pdflatex zhang-collab
	pdflatex zhang-collab

show_nt: pdf
	- killall AcroRd32 
	cp main.pdf main_$(MY_DATE).pdf
	$(ACROREAD) $(PREFIX)main_$(MY_DATE).pdf &

clean:
	rm -rf *.aux *.log *.bbl *.blg *.out $(PDF_TARGETS)





==> api-bak.tex <==
\section{API-Augmented LLMs}
\label{sec:study}

This section first discusses popular API-augmented LLM frameworks and then presents properties of typical APIs from our empirical study.

\subsection{API-Augemented LLM Frameworks}

%\yiying{talk about each framework's implication on inference system and briefly on how they improve the quality of LLM answers}

To extend LLMs' ability to undertake more types of tasks, various approaches have been proposed to {\em augment} an LLM with tool, or API, uses. Below, we briefly describe typical API uses in two broad categories.

The first type of APIs are non-LLM tools called during the decoding phase of an LLM, usually aimed to extend the type of tasks the LLM can handle. These APIs range from simple tools like calculator~\cite{XXX} and calendar~\cite{XXX} to real-world interactions like information retrieval~\cite{XXX} and restaurant reservation~\cite{open-table-chatgpt-plugin}. Additionally, an API can invoke another machine-learning model such as translation~\cite{XXX}, query-answer (QS)~\cite{XXX}, text-to-speech generation~\cite{XXX}, and image generation~\cite{XXX}.
An LLM is usually fine-tuned to generate appropriate API calls automatically during the decoding phase, with frameworks like TaLM\cite{parisi2022talm}, ToolkgenGPT\cite{hao2023toolkengpt}, and Toolfromer\cite{schick2023toolformer}.

The second type augments a single LLM call by making multiple calls to the same LLM or to other tools. For example, to have contiguous interaction with a human, a chatbot can take rounds of back-and-forth chats by calling an LLM at each step and maintaining a history of chat~\cite{XXX}. Similarly, LLMs can be augmented to interact with a virtual environment by taking actions and reacting to action results in the virtual world in steps~\cite{XXX}. Apart from these use of multiple LLM calls, another popular use case is to decompose a complex task into multiple steps. For example, Chain-of-Thoughts~\cite{wei2022chain,XXX} break one request into a chain of ``thought'' steps, each being a new prompt to an LLM that continues the history of thoughts. Similarly, ReAct~\cite{yao2022react} uses a chain of reasoning and action to accomplish complex tasks. To assist users in expressing such augmented LLM usages, LangChain~\cite{LangChain} and Gorrila~\cite{Gorrila} provide programming models for users to trigger LLMs or tools in a task flow.  
%Recent works have described Augmented Language Models(ALM) that can take advantage of outside information in order to provide more factual information without hallucinations\cite{Augmented Language Models A Survey Paper}. The approaches for these techniques can be split into better prompt reasoning decomposition, tools act, and model based. 

%CoT\cite{wei2022chain}/ReAct\cite{yao2022react} are few shot prompting techniques that aim to provide example prompts with intermediate steps. The language model is repeatedly called to improve the model's ability to decompose problems and reason. These approaches can be used to perform API calls that provide outside information such as calculator, wikipedia, etc. Some tools such as Gorrila/Langchain aim to use tools using this strategy. 

%Works such as TaLM\cite{parisi2022talm}/ToolkgenGPT\cite{hao2023toolkengpt}/Toolfromer\cite{schick2023toolformer} aim augment the model's performance by providing the task of when to call an API to the model itself. Toolfromer, for example, does this by finetuning a model with the a list of apis provided by RapidApi\cite{rapidapi}. 

\input{tbl-api-study}
\input{fig-api-study-1}

\subsection{API Calls and Their Properties}

%\yiying{We should organize this section by API domains/categories. For each domain, we talk about what the API is doing and then present its execution time CDF, number of calls, context lengths (not sure about return length as we are currently not doing anything on it). At the end summarize the key takeaway of all these API types.}

%We analyze the properties of different datasets to evaluate the effectiveness of our inference system. We consider datasets from arithmetic, a knowledge-based question and answering system, a multi-step chat bot, and an embodied virtual environment. The dataset demonstrates different execution time, frequency of API calls, and context lengths. We augment the datasets with relevant APIs from calculator, wikipedia, and a virtual environment gym.

To understand LLM APIs and design inference systems for them, we first examine a set of representative APIs, including arithmetic (math), question-and-answer (QA), virtual environment (VE), chatbot, image generation, and text-to-speech (TTS), to answer three key questions: 1) how long does an API call take? 2) how many API calls are generated for a request?, 3) what is the context length when an API call is made? 
We leave other metrics like API returned token length, detailed CDF distributions, and our evaluation methodology to the Appendix, and 4) how many tokens are returned from an API call?
%

We profile these workloads on a server with one A6000 GPU and an Intel(R) Xeon(R) Gold 5218 CPU, and we use Vicuna~\cite{vicuna2023} as the LLM. We trigger the math, QA, and VE APIs using the ReAct~\cite{yao2022react} framework. ReAct uses an event loop of observation, action, and response by prompting an LLM with corresponding instruction prompts. %Here, we prompt Vicuna to use APIs. %We model the ReAct event loop with a server running the Vicuna LLM model~\cite{vicuna2023} and a client interacting with the model to perform multiple calls. 
%The exact number of ReAct calls and execution time might vary from system to system, but our profiling emulates a potentially realistic workload. 
% \yiying{what's your methodology for the three long APIs}
For the Chat API, we directly use the conversations from the ShareGPT dataset~\cite{vicuna_share_gpt}.
For the Image and TTS API, we use GPT-4 prompting in order to create a dataset with multiple calls.
%We measure the API execution time, the number of API calls, the number of returned tokens of an API call, and the context length when an API is called.
Table~\ref{tbl-api-study} summarizes our results with average values. %Overall, the six APIs can be categorized into short-running and long-running ones. 
Figures~\ref{fig-api-study-1} and \ref{fig-api-study-2} present the detailed CDF results the four metrics for short-running APIs (math, QA, VE) and long-running APIs (chatbot, image, TTS).
Below, we briefly introduce each API type and discuss their properties.

%\input{fig-api-study-2}


\boldunderpara{Arithmetic (Math).}~~~ 
LLMs struggle to perform complex mathematical reasoning due to these operations' explicit representation and manipulation, giving rise to the use of arithmetic APIs. We evaluate arithmetic-API-augmented LLM by prompting Vicuna with instructions on taking reason and action step by step (\ie, following the ReAct method) to solve each arithmetic problem, where the action is calling a Python calculator API.
We evaluate this arithmetic-augmented Vicuna using the GSM8K-XL~\cite{hao2023toolkengpt} dataset, which contains 8.5K high-quality grade school math problems created by human problem writers. As expected, calculator APIs' execution times are short, with an average of 0.2 milliseconds. It has a fairly large context length when APIs are called because the ReAct-way of instruction prompts are long. %This implies that the majority of the workload is dominated by normal decoding.

\boldunderpara{Knowledge-based question and answer (QA).}~~~ 
Pre-trained LLMs lack the ability to access knowledge beyond their training dataset. % and can suffer from hallucinations and factual errors. 
One way to mitigate this issue is to augment LLMs with knowledge-based QA, where information is retrieved from a rich dataset to answer questions. %It augments queries with information retrieved from a dataset to provide better contextual information to users. 
%LLMs can be augmented with knowledge-based QAs to provide better answers with less hallucinations.
%Using retrieved information can reduce the effect of factual errors and hallucinations.
To understand this augmentation, we use the Multihop QA Wikipedia~\cite{yang2018hotpotqa} dataset, which consists of questions requiring multiple calls to search in Wikipedia. We use the ReAct framework to prompt the LLM to call a Wikipedia endpoint with different questions. %The responses from the Wikipedia endpoint are postprocessed. We use the live Wikipedia API endpoint for our benchmark and 
For each call, we retrieve a summary of the relevant Wikipedia page, which we post-process by limiting the size of the responses to fit within the maximum model sequence length. This knowledge-based QA API has a longer context length because of the question nature. Its execution time is relatively short but highly varied because of the non-deterministic network communication latency. 
%The return length is shorter than real answers because of the maximum sequence length supported by Vicuna. With a larger model with a higher maximum sequence length, we expect more return tokens from QA. 


% \yiying{which LLM? also Vicuna? if all experiments are using Vicuna, we should just say that in the beginning of sec3.1. I added it end of section 3.1} 

% \yiying{what is 11prompted wiki page''. Meant what was returned by LLM?}
%\fixme{how is it integrated with LLM}
\boldunderpara{Virtual Environment (VE).}~~~ 
Recent works have tried to use language models to control and interact with embodied agents in virtual environments~\cite{Gu_2022, huang2022language, hu2023look}. 
Accomplishing a complex task in virtual environments usually involves multiple gradual steps, each being one VE API call.
%However, LLMs may struggle to learn the environment and provide actions that are grounded.
%Previous work, such as ToolkenGPT~\cite{hao2023toolkengpt} and BUTLER~\cite{shridhar2020alfworld}, uses API calls to augment the LLM. We use the ALFWorld dataset~\cite{shridhar2020alfworld} %that contains a list of household activities to perform in an interactive embodied text environment.  
To evaluate VE APIs, we use the ALFWorld dataset~\cite{shridhar2020alfworld}, an interactive environment that aligns text descriptions and commands with physically embodied robotic simulation.
Specifically, we prompt the Vicuna LLM with an initial virtual environment and use the ReAct event loop to repeatedly interact with the environment. This VE API has a short execution time due to a locally executed embodied text-based environment. A vision-based VE API would potentially incur a longer execution time. %The VE API also returns a short response because each interaction with the environment is fairly simple, such as `pick up`, `go`, and `open`. The context length is long because of the long initial instruction prompt.


\boldunderpara{Chatbot.}~~~ 
A popular task for LLMs is a chatbot, which interacts with human with a sequence of chats. Here, we view human responses as an API, as the time human uses to respond essentially leaves, or {\em preempts}, regular LLM processing, but the chat history %(what the LLM has already processed and generated) 
should be kept as a context for following chats. 
%Although this augmentation to LLMs does not call any actual computing function, the nature of the human-response API is the same as computing APIs. 
To evaluate chatbots, we use the ShareGPT dataset~\cite{vicuna_share_gpt}, which contains crowd-sourced real-user ChatGPT conversations. 
As ShareGPT does not provide information of human response time, we estimate it (\ie, the API execution time) as the summation of the reading time of previous chat response and the writing time of the next prompt. We estimate these times by the average human reading~\cite{brysbaert_2019} and typing~\cite{ma2015haptic} speed multiplied by the number of response and prompt tokens.
All other metrics reported are from ShareGPT. The context %and return 
lengths vary greatly due to the variety of human chats and chat generation. With our way of estimating human response time that is proportional to chat lengths, the ChatBot API's execution time also has a high variation. %This necessitates an algorithm that dynamically handles this variance. 
%Table~\ref{tbl-api-study} and Figure~\ref{fig-api-study-2} present the 
%We simulate multiple rounds of conversation as an api call that takes a certain amount of time and responds. 
%The execution time of the chatbot provided is synthetic. We use the reading time of the prompt * average reading speed + writing time * average reading speed in order to . However, the number of calls for the chatbot is the number of calls in an actual conversation trace from ShareGPT dataset.


\boldunderpara{Image Generation.}~~~ %Image generation is a complex task requiring substantial compute and memory access. 
In recent years, generating images from language descriptions has become a popular AI task. 
An LLM can be used to facilitate a sequence of image generations. 
A human can gradually describe the features of an image based on observations from generated images. For example, a user might generate an image of a face and incrementally describe features around the face to get the desired image. Under this use case, an LLM calls two types of APIs, one for image generation and one for waiting for the next prompt from a human. The latter API type is the same as the one in Chatbot.
%Recent works have combined text prompts with Image generation to provide a better image-generation experience. 
To understand image-generation-augmented LLMs, we create a dataset by generating a series of image-generation prompts using GPT-4-based ChatGPT. We prompt GPT-4 to generate complex Stable Diffusion prompts at a certain size. Each prompt will trigger an API call of the Stable Diffusion model~\cite{stable_diffusion} to generate an image. %Each round with the LLM involves a user prompt with normal decoding and then a diffusion call. The number of calls total is modeled around the chat dataset.
We estimate the number of image generation rounds (\ie, number of API calls) to be the same as the number of chatting rounds in Chatbot. 
%As there is no standard way of returning tokens from an image generation, we use a short, constant-length sentence describing the generated image as returned tokens. 
For API execution time, we measure the actual Stable Diffusion call and estimate the human response time in the same as as Chatbot; the sum of them at each round is shown in Table~\ref{tbl-api-study} and Figure~\ref{fig-api-study-2}. %For the context and return length, we provide a mixture of ShareGPT dataset~\cite{vicuna_share_gpt} and the real prompts. 
The execution time of the image generation API has high variation due to variations in executing a diffusion model and the variation in human responses. 
The %return and 
average context length is shorter than the Chat API due to smaller input prompts to the diffusion API. %The context length and return length variance is directly due to the variance in huamn responses in the ShareGPT dataset. 


\boldunderpara{Text-To-Speech (TTS).}~~~ 
Text-To-Speech converts text to speech. As demonstrated by the ChatGPT Whisper API support~\cite{chatgpt-whisper}, TTS can be integrated with an LLM to make conversations with a human. We use a methodology similar to image generation to understand TTS-augmented LLMs. Specifically, we use ChatGPT to generate a series of prompts, which are then sent to the Vicuna LLM. Each prompt triggers an API call to the Bark TTS model~\cite{tts_sunoai2023bark}. Similar to image generation, we estimate 
%API return length and 
the human response time but measure actual TTS execution time. 
TTS's behavior is similar to image generation, with high variation in API execution time due to variations in model execution time and user response time.  


 

% \boldunderpara{API overview.}
% talk about the types of APIs out there and the ones we study
%We run a ReAct~\cite{yao2022react} on these datasets to categorize the performance of these different Apis on LLMs. Our run was on a a100 on AWS.
%We summarize the properties of the API in table \ref{table:api_properties}. 

%We also provide the distribution of number of api calls per dataset for using CoT/ReAct methodoly. Extended CDF distributions of different properties such as execution time are provided in Figures \ref{fig:cdf_api_properties_short},\ref{fig:cdf_moderate}.

\boldunderpara{Summary and Insights.}~~~
Overall, we find API execution time to be highly dependent on API types and exhibit a clear difference between short-running (Math, QA, VE) and long-running (Chatbot, Image, TTS) ones. APIs that are fully automated with no human interaction are usually short and exhibit small variations (other than QA, which interacts with the network). 
On the other hand, APIs that involve human interaction and/or calling another large machine-learning model are long-running. They exhibit a high variation in execution times because of the non-deterministic nature of humans and large models. 
The short/long execution times and their variation imply that no single API preemption strategy is universally applicable, but an inference system could utilize API type as a hint of execution time features.

The number of API calls in a request and API return lengths are overall small across workloads, while the context lengths are significantly larger. Long context lengths imply that the amount of GPU memory wasted (because of preserving, recomputation, or swapping) is significant, emphasizing the importance of a good preemption strategy. Meanwhile, it means that the model still spends most of its time performing prefill and normal decoding, with little computation needed for processing API-returned tokens. 

%This necessitates a dynamic scheduling/pre-emption policy over a fixed heuristic. 



==> design-bak.tex <==
\section{\sys\ Design}
\label{sec:design}
In this work, we build an LLM serving system, Vulcan, that supports extensive augmented LLM models and develop a new scheduler that addresses the issues outlined in \ref{sec:study}. The high-level overview of Vulcan is depicted in \fixme{xxx}. Vulcan implements preemptive scheduling for sequences making API calls, i.e. paused requests, and employs a novel algorithm to estimate the cost/benefit of preemption. Specifically, we propose to use \textit{GPU resource waste}, which stands for unused GPU memory over a certain amount of time, as the estimation criteria. In each forwarding iteration, our scheduler selects a subset of paused sequences as the preemption targets according to the estimated waste, then passively preempts them as needed.

In the following sections, we first articulate the scheduling algorithm in \ref{sec:alg}. Then we describe our optimized preemption mechanism that jointly considers evicting and discarding KV caches of paused sequences in \ref{sec:fpreempt}.

\subsection{Overall Algorithm}

first decide preserve or not preserve, based on whether memory spent on preserving context is higher or lower than memory wasted because recomputation overhead

Then for the not preserve requests, rank them by recomputation memory waste.

Then we swap from the highest discard waste request as much as we can (until the swap limit). if swap limit not hit, go to the next hightest disacrd waste request. and so on.

Swap limit is decided by the batch size. batch size is determined by the batch formation: number of running requests plus number of waiting requests that we can add without crossing the compute saturation point or GPu memory space. compute saturation point (beyond that no improvement of throughput)

API return time. at each iteration, swap in as much as the swap limit allows. swap requests based on FCFS (request arrival rate). 

swap in and swap out are serially executed
swap out vs swap in split of bandwdith: solve linear equation at static time by
maximizing swap in tokens + scheduled batch tokens, while ensuring:
1. swap in tokens + scheduled tokens <= swap out tokens + free GPU memory
2. swap in time + swap out time <= iteration time (iteration time profiled)
3. swap out amount - swap in amount <= free CPU memory
assuming at each iteration there are always plenty tokens to swap in and to swap out 

kernel used for attention computation from scratch (no kv cache available): use xformer 
otherwise, use deepspeed kernel. for multi query, parallelize queries with flashattention.

First, we reason about GPU memory by assigning a decision for each paused request. This is done by computing a waste term for each decision: preserve, discard, and swap. The decision with the least waste is selected. We formulate waste as a unit of memory-time. The waste from preserving a request is straightforward: for as long as a request is blocked on its API call, it occupies memory that cannot be accessed by running requests. The waste from discarding/swapping a request comes from having to recompute/swap its context; this adds latency to the recomputation iteration, which wastes memory occupied by running requests. In essence, eviction adds pure time to an iteration which instead could have been used to execute more iterations of the running group.

The preserve waste of request $i$ is equal to the API execution time $api_i$ multiplied by its context length $c_i$ (or the memory it occupies).
\begin{equation}
preserve_i = api_i * c_i
\end{equation}

To obtain the recomputation waste, we profile the model and hardware to model the relationship between the number of query tokens in a batch and the corresponding model forwarding time. We denote this term as $f(x)$ where $x$ is the number of tokens in the batch. The unique latency added by recomputation is $f(c)$, and the memory wasted during this time is the sum of all memory utilized by the running group $R$.
\begin{equation}
discard_i = f(c_i) * \sum^R_r c_r 
\end{equation}

Finally, we also profile the per-token swapping latency, and denote this as $s(x)$ where $x$ is the number of tokens that are swapped. Since memory needs to be both swapped in and out, this term is multiplied by 2.
\begin{equation}
swap_i = 2 * s(c_i) * \sum^R_r c_r
\end{equation}

While we do not know the true size of the running group, we observe that the amount of memory consumed by the running group stabilizes once the system is in a steady state. Once each of these terms is computed for all paused requests, we select $\textbf{argmin}_i \{preserve_i, discard_i, swap_i\}$ for each request.

To decide between requests in the waiting queue (either new or previously discarded) and requests that can be swapped in (previously swapped), we use FCFS.


\label{sec:alg}

\boldunderpara{API execution time.}
1) The longer an API executes, the more memory*time we can potentially reuse. => We should favor discarding tokens from longer-running APIs like chatbot over short-running ones like calculator, so as to increase the ratio of <memory (size*time) saved>/<recomputation needed>
2) API calls have different execution times. Some API types like calculator have predictable (stable) execution time, while others are unpredictable (\eg, when a user responded in a chatbot). => For predictable API times, we can give priority to short ones when choosing requests to discard/swap blocks. For unpredictable API times or for adjusting for wrong predictions, we need a dynamic way to adapt the priority of a request in terms of block discarding and swapping.
3) For predictable API time requests, we can explore the possibility of pre-recomputing of earlier tokens just in time before the API returns.

maintain three request queues: running, paused (API calls being made or normal requests intercepted), and waiting (new requests waiting to start).
For each request, we track its context length and the number of tokens being cached in kv cache.

two types of memory blocks: active (those currently being used by running requests) and inactive (not currently used). For inactive blocks, we first group them by their corresponding requests' API call remaining time. Then, within each group, we sort blocks by their positions in the corresponding sequence (from earliest to latest).

When an API call is triggered, we add its context (current cached KVs) to the corresponding inactive block group based on the API type. Here, we assume that we can estimate the API call time based on the call type and input to the call, we will discuss how we deal with unknown API call times in \S\ref{sec:unknown-api}. 
We round robin requests within the longest-running API group for K rounds by swapping out earliest tokens. Then round robin the second longest-running API group for K rounds, etc. If we run out of blocks from API groups, we need to swap/discard regular blocks from non-API running requests, and we add these blocks to the inactive block group with API time zero, \ie, the bottom group.

When an API returns or when there is room for a paused non-API request, we need to swap in or recompute discarded tokens of it plus computing the API returned tokens (for API requests). \fixme{mechanism for recomputation to be filled.}

% \input{fig-transformer-block}

\boldunderpara{Getting $f(x)$}
To accurately determine the iteration time, the first question to answer is: what independent variables can control the workload of a full model forwarding pass? From our profiling results, we find that linear layers and attention layers account for nearly \emph{95\%} of the total execution time of the transformer block. Thus we only study the behaviour of these operations in this work.

The linear layers apply matrix multiplication to all input tokens, meaning its computation complexity scales linearly to the batch size. If a batch contains one request processing its prompt tokens, all tokens from that sequence will be forwarded in that iteration, which results in a large batch size that can easily saturate the GPU utilization. In this case, the mapping between the batch size and the layer execution time would be highly accurate. However, this is not always true, as the number of inflight tokens can be arbitrarily small because of the limited GPU memory capacity. For example, if all requests in a batch are performing normal decoding, the device memory would have to hold the KV value for all history contexts to generate a new token. This small batch size leads to memory-bounded computation if not fully occupying streaming multiprocessors, which adds complexity to our mapping function to describe this behavior. Existing works such as \fixme{add deepspeed and chunk-prefill paper} propose to fuse prompt stage sequences with normal decoding ones in each iteration to stabilize the number of inflight tokens. We also adopt this technique to maintain a reasonably large batch size across iterations so that our function only needs to cater to more predictable scenarios. More details about our chunking policy can be found in Sec\fixme{add text for our prefill-chunk, include profile, conservative scheduling to prevent looking far into future. }

Additionally, we study the performance of self-attention kernel, which takes QKV matrices of input sequences and computes the attention score for each query. This kernel can contribute more than \emph{50\%} of the overall forwarding time when most of the sequences in a batch are in the normal decoding phase. Thus, it is equally important for our estimation function to capture its behavior when predicting the model runtime. In attention operation, each sequence will calculate its attention score separately but concurrently. The computation complexity and the amount of memory access can depend on the number of queries and sequence length for each sequence, which creates a group of tasks with ragged workloads competing for GPU resources. Instead of mapping from the fine-grained batch composition to the kernel performance, we find that the execution time of the attention kernel stays consistent if the running workload requires the same amount of device memory, which is always the case in a production environment where the GPU memory is fully occupied by the KV cache. \fixme{add arithmetic plot for arith intensity} This finding aligns with the fact that attention calculation is heavily memory-bounded because of its low arithmetic intensity. This also remains true even with the adoption of FlashAttention implementation.

Combining these two insights, we choose to build our iteration time predictor around a single factor: the total number of inflight tokens in the batch. We perform offline profiling on the given GPU hardware and fit a linear model that maps the batch size to the model forwarding time. Specifically, we 

%We first need to decide how many tokens to recompute/compute within each iteration, based on batch size to achieve good throughput for the mixed decoding-recomputation iteration, while controling request latency. Then, for each iteration, we check if there's enough GPU memory. If not, we trigger the discard algorithm above.

\subsection{Faster Preemption}
\label{sec:fpreempt}
The naive implementation of swap will add significant overhead. As each memory region needs to launch a CUDA kernel for swap, kernel launching time could dominate the swap latency. As swap out and swap in both block computation (swap out blocks the memory to be freed and used by other requests, swap in blocks the returning API request), swap with naive implementation would significantly slow down the whole process.

We design a swap scheme to fully overlap swap kernel launching and data movement in a layer-by-layer pipeline way.

\subsection{Dealing with Unkonwn API Time}
\label{sec:unknown-api}

==> design-old.tex <==
\section{\sys\ Design}
\label{sec:design}

built on top of iteration-level scheduling and paged attention

\subsection{Design Building Blocks}

\boldunderpara{Preserve.}
Preserving a request's context during its API calling time has the advantage that upon the API return as the request can resume immediately. However, the memory used for maintaining the context is wasted during the API call time. Longer API call time and longer context cause more memory wastage.

\subsubsection{Optimizing Swapping}
1) CPU swap memory space is mostly not the bottleneck
(144GB CPU memory per GPU on p4d instance).
% \fixme{add calculation of how much memory would be needed for a certain model size, API length, and batch size}
Consider llama-13B, hidden\_size: 5120, num\_layers: 40, type: FP\_16, all sequences of length 2048 tokens. %A CPU memory of space 1\TB\ can accommodate 655 sequences.
With a mixed API time (uniform sample from 0.1s to 20s) workload, average 18 APIs made for each API, the maximum swap space needed is 127.4\GB.
2) Naive implementation of swap will add significant overhead. As each memory region needs to launch a CUDA kernel for swap, kernel launching time could dominate the swap latency. As swap out and swap in both block computation (swap out blocks the memory to be freed and used by other requests, swap in blocks the returning API request), swap with naive implementation would slow down the whole process significantly.
=> We design a swap scheme to fully overlap swap kernel launching and data movement in a layer-by-layer pipeline way.
3) Even with optimized swap, the swap bandwidth can still be the bottleneck when the number of tokens to be swapped out/in exceed the PCIe link bandwidth. From results shown in Table~\ref{tbl-free-swap}, swap alone is usually not enough for API calls, esp. when a server has more GPUs competing for PCIe bandwidth, which is a common case for server environments.
=> Swap can be treated as ``free'' until a certain number of tokens, and we should always swap out these many tokens first.
4) Swap out and swap in both consume PCIe bandwidth. 
=> At each iteration, we need to decide how much bandwidth to give to swap out (API-calling requests) and to give to swap in (API-returning requests). The former improves throughput, and the latter improves request latency (SLA).
%=> \fixme{get the comparison between preserve, swap, and discard (recomputation) on p4d (A100) and our machine (A6000)}
%=> \fixme{getting tradeoff of swap speed (kernel launching speed) vs. block size}

\fixme{Need a figure with x axis number of tokens swapped and y axis performance slowdown (compared to no swap). should see a turning point for each config}

\fixme{need a figure to illustrate how we overlap swap with computation}

\input{tbl-free-swap}

\subsubsection{Optimizing Discard and Recompute}
\boldunderpara{Discard and recompute.}
Apart from preserving and swapping, we can also discard context and recompute it for API requests to resume after their API calls finish.
1) How much to discard: We observe that most server-grade GPUs have unused computation resources (GPU cores) when their memory space is saturated for running LLMs.
Thus, in each iteration, we can add the recomputation of a certain number of discarded tokens without delaying the iteration, as the recomputation of context involves a higher compute-to-memory ratio than normal decoding. 
=> can discard these number of blocks almost for free, but beyond that we will cause GPU resource wastage in an iteration for other requests to wait for the recomputation (straggler) to finish.
2) When to recompute: To avoid stragglers, we can chunk discarded tokens to be computed in multiple iterations. However, chunking will make the API request's latency longer and potentially violate SLA (which is usually expressed as token generated in a second for a request).
=> We can chunk discarded tokens (and API returned tokens) as much as we need (for avoiding straggler) unless it violates SLA.
3) What blocks to discard within a request: The earlier a recomputed token is in a sequence, the less GPU memory is required for the same amount of compute. Earlier tokens can be computed separately without the need to load any context.
\textbf{Proof of 3):}
Let $t$ be the number of API return tokens, $c$ be the context length of the sequence, $h$ be the hidden size, $e$ be the number of evicted tokens, and $p$ be the number of preserved tokens. We are guaranteed that $c = p + t + e$ and that $t > 0$. Discarding from the front and back both result in a query size of $t+e$. The performance of non-attention operations is the same because it is a function of the number of query tokens. During attention, a token attends to all previous tokens in the sequence. Discarding from the front results in the following computation for $Q@K^T$: $(e,h) @ (h,e) + (t,h) @ (h,c)$. The total FLOPs are $2e^2h + 2thc$. Discarding from the back results in the following computation for $Q@K^T$: $((e + t),h) @ (h,c)$. The total FLOPs are $2ehc + 2thc$. $2e^2h < 2ehc$.

\fixme{Need a figure with x axis number of tokens discarded and y axis performance slowdown (compared to no discarding). should see a turning point for each config}

\fixme{need a figure to show the effect of chunking, probably also a figure to compare front of sequence and back of sequence for discarding}

\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{ |c|c|c|c|}
\hline
 workload & Context Len & A6000-48GB & A100-40GB \\
 \hline
  {GPT-j-6B, total seq} & 256 & 256 & nan \\
{GPT-j-6B, free recomp} & 256 & 64 & nan \\
\hline
{GPT-j-6B, total seq} & 512 & 137 & 87 \\
{GPT-j-6B, free recomp} & 512 & 53 & 41\\
 \hline
 {GPT-j-6B, total seq} & 768 & 91 & nan \\
{GPT-j-6B, free recomp} & 768 & 37 & nan \\
\hline
% GPT-j (6b, 512) & 112, 16 & 87, 41 \\
{GPT-j-6B, total seq} & 1024 & 69 & 44 \\
{GPT-j-6B, free recomp} & 1024 & 59 & 84\\
% GPT-j (6b, 1024) & 56, 72 & 72, 84 \\
 \hline
 {baichuan-13B, total seq} & 1024 & 17 & nan \\
{baichuan-13B, free recomp} & 1024 & 111 & nan\\
\hline
\end{tabular}
\mycaption{tbl-free-recomp}{``Free'' recompute tokens.}
{The maximum number of tokens that can be freely recomputed in each iteration highly depends on the hardware limit and the workload. We set a fixed length for all sequences and a batch size that can saturate GPU memory.}
\label{table:api_properties}
\end{center}
\end{table}

\begin{figure}[!htb]
\centering
\includegraphics[width=\columnwidth]{Figures/free-recomp.png}
% \vspace{-15pt}
% \caption{The figure describes the distribution of api calls within dataset. Different requests might require a different number of api call and execution time. This requires a smart scheduling and eviction system. }
\label{fig:free-recomp}
% \vspace{-15pt}
\end{figure}

\boldunderpara{Inter- and intra-request block choices.}
1) Recomputing or swapping in shorter sequences allows for a request to be resumed sooner.
2) The recomputation of tokens from different requests can all be placed within one iteration, while the recomputation of tokens within a request have to be sequentialized. 
Because of 1) and 2), we want to discard or swap earlier tokens in multiple paused requests instead of from one single request. 
=> Idea: treat all the requests of similar API time as the same and get blocks from any of them (but start from the beginning).

\fixme{My current impression is that this is not significant. but if it is, we should show a figure comparing inter and intra request discarding}

\boldunderpara{API execution time.}
1) The longer an API executes, the more memory*time we can potentially reuse. => We should favor discarding tokens from longer-running APIs like chatbot over short-running ones like calculator, so as to increase the ratio of <memory (size*time) saved>/<recomputation needed>
2) API calls have different execution times. Some API types like calculator have predictable (stable) execution time, while others are unpredictable (\eg, when a user responded in a chatbot). => For predictable API times, we can give priority to short ones when choosing requests to discard/swap blocks. For unpredictable API times or for adjusting for wrong predictions, we need a dynamic way to adapt the priority of a request in terms of block discarding and swapping.
3) For predictable API time requests, we can explore the possibility of pre-recomputing of earlier tokens just in time before the API returns.

\if 0
\boldunderpara{API returned sequence length.}
1) API calls can return different number of tokens, and these tokens need to be processed before going back to normal decoding. Longer returned length the more new tokens we can ``generate'' per second (for SLA). 
=> We can afford discarding more tokens if we anticipate long return length.
2) For some API types like calculator and calendar, we can predict the return length, while for others, we can only know the maximum possible return length (smaller than max sequence length supported by the model).
=> \fixme{??? what to do here}

\boldunderpara{Batch composition.}
At any iteration, there can be requests doing normal decoding, having new API calls, and returning from API calls. There can also be new waiting requests and paused running non-API requests because of being out of memory. A batch's composition determines 1) how much swap out vs swap in, 2) how much computation could be given to recomputation and normal decoding/prefill, and 3) how many tokens we could potentially generate if given a certain amount of more memory. While the current batch's composition is known, we need to anticipate a future batch's composition (when an API returns) to make the decision at API call time.
=> Historical (weighted average) based batch composition estimation. Simplifies the design.
\fi
%\boldunderpara{Tail latency and SLA considerations.}

\subsection{Strawman Designs}

Before presenting our final design, we discuss two strawman designs that are also derived from our study results and are seemingly feasible.

\subsubsection{Strawman 1: Heuristic-Based}
Our first strawman design uses heuristics to decide whether a request should be preserved, discarded, or swapped. 

\subsubsection{Strawman 2: Optimization-Based}

\subsection{Full Design}

putting everything together:
It boils down to 1) how to best utilize GPU memory, 2) how to best utilize GPU compute, and 3) how to best utilize swap bandwidth, for better throughput while meeting SLA.

Preserve:
No memory usage and no recomputation/swap.

Swap:
Memory usage: + tokens generated with amount of memory swapped out * API call time
Memory waste: - tokens that could have been generated if not waiting for swap = tokens generated with remaining of GPU memory * waiting time
Latency overhead: - number of chunking iterations or time to swap in everything within an iteration

Discard:
Memory usage: + tokens generated with amount of memory discarded * API call time
Memory waste: - tokens that could have been generated if not waiting for recomputation = tokens generated with remaining of GPU memory * waiting time
Latency overhead: - number of chunking iterations or time to recompute everything within an iteration

maintain three request queues: running, paused (API calls being made or normal requests intercepted), and waiting (new requests waiting to start).
For each request, we track its context length and the number of tokens being cached in kv cache.

two types of memory blocks: active (those currently being used by running requests) and inactive (not currently used). For inactive blocks, we first group them by their corresponding requests' API call remaining time. Then, within each group, we sort blocks by their positions in the corresponding sequence (from earliest to latest).

When an API call is triggered, we add its context (current cached KVs) to the corresponding inactive block group based on the API type. For unknown API types, we add their blocks to \fixme{???}.  We preserve the API blocks if API call time is less than \fixme{???}. Otherwise (say we need $k$ blocks to continue running \fixme{or to run new requests???}), we decide whether to swap $k$ blocks to CPU memory or to discard them based on the following. \fixme{to be filled} If the decision is to discard, we discard blocks based on the following policy. 

where $B$ is batch size, $n_d$ is number of discarded chunks, $n_s$ is the number of swapped chunks, $s_x()$ is a function that measures swap latency given a number of chunks, $t$ is number of tokens in API return, and $d$ is a constant for model forwarding duration.

FIXME: $B$ and $d$ are currently treated as constants. However, $d$ can significantly change the result. We should fix this

We round robin requests within the longest-running API group for K rounds by discard earliest tokens. Then round robin the second longest-running API group for K rounds, etc. If we run out of blocks from API groups, we need to swap/discard regular blocks from non-API running requests, and we add these blocks to the inactive block group with API time zero, \ie, the bottom group.

When an API returns or when there is room for a paused non-API request, we need to swap in or recompute discarded tokens of it plus computing the API returned tokens (for API requests). \fixme{algorithm/policy for recomputation to be filled.}
%We first need to decide how many tokens to recompute/compute within each iteration, based on batch size to achieve good throughput for the mixed decoding-recomputation iteration, while controling request latency. Then, for each iteration, we check if there's enough GPU memory. If not, we trigger the discard algorithm above.

==> design.tex <==
\section{\trick}
\label{sec:design}

This section presents min-waste preemption, or \trick.
We first present how \trick\ optimizes swap by completely hiding its induced memory waste. We then discuss how \trick\ reduces recomputation memory waste of \discard. With these improved techniques, we present how we calculate the memory waste of every API call and how we make preemption schedules within and across API requests. Finally, we discuss how we deal with unknown API execution time.
%The core idea of \trick\ is to minimize 
%adaptively choose a hybrid of discard, preserve, and swap within and across requests making API calls based on a GPU memory waste estimation. 
%, the first inference system designed for API-augmented LLMs. 
%To efficiently support API-augmented LLMs, an inference system should solve several challenges. 1) When an API call is triggered, how to decide whether to discard, preserve, swap out the request's context or a combination of them? 2) With limited swap bandwidth and recomputation budget, how to decide which requests to discard or swap out first? 3) How to determine 
%This section presents how \sys\ solves each of these challenges.

\subsection{Offline Profiling}
We conduct a profiling step where we determine two important relationships: $T_{forward}$ and $T_{swap}$. $T_{forward}$ is a function that maps the number of scheduled tokens in a batch to the execution time of that iteration, obtained via curve-fitting. $T_{swap}$ similarly maps the number of tokens scheduled to be swapped to the swap latency, and can be exactly computed based on the swapping bandwidth and the per-token memory requirements. Each model deployed on a specific hardware setup will have a unique set of equations that can be obtained accurately offline. Both are linear functions. 

$T_{forward}$ displays a strong relationship to the number of input tokens but is largely agnostic to the context length of each sequence. This is because the linear layers are solely proportional to the number of input tokens, while the attention layers that compute over the context is memory-bounded. We also find that $T_{forward}$ is a piecewise linear function that has two parts. As the number of input tokens approaches the boundary, the throughput will continue to increase. Once it crosses the boundary, its throughput will remain constant. We call this boundary the \textit{saturation point}, as it represents the point where the GPU compute is fully saturated. We utilize these relationships to optimize swapping and recomputation.

\subsection{Swap Pipelining and Chunking}
\label{sec:improve-swap}

We now discuss how \trick\ avoids swap memory waste.
%Before presenting \trick's full algorithm, we first introduce how we optimize \discard\ and \swap\ to reduce GPU memory waste and improve performance, as our overall algorithm uses the optimized versions when making various decisions.

%The naive implementation of swap will add significant overhead. As each memory region needs to launch a CUDA kernel for swap, kernel launching time could dominate the swap latency. As swap out and swap in both block computation (swap out blocks the memory to be freed and used by other requests, swap in blocks the returning API request), swap with naive implementation would significantly slow down the whole process.

\boldunderpara{Swap pipelining and overlapping.}~~~
% We can say less in this part to save space. the optimization itself is straightforward
The naive implementation of \swap\ launches all memory copy kernels at the beginning and blocks computation until the data movement finishes. The memory copy overhead is then proportional to the number of tokens to swap, which can be a noticeable portion of the iteration time. Moreover, with PagedAttention~\cite{vLLM}, the context of an API request can scatter across many physical memory regions (blocks), leading to exceedingly more swapping kernels to launch which further delays the scheduling of the following computations. We optimize the KV cache transfer by pipelining the swap task. Specifically, after the kernel launching process at each layer, we trigger an asynchronous transfer of KV values for the next layer. The pipelined swapping overlaps the kernel launch overhead and the actual data movement with normal computations. % Add real number if needed
%Apart from affecting iteration time, t
% The naive implementation of \swap\ has a major performance bottleneck: each memory region in the context requires the launch of a CUDA kernel for data movement. With PagedAttention~\cite{vLLM}, the context of an API request can scatter across many physical memory regions. Thus, swapping context memory could take extremely long, causing GPU memory waste for other running requests to wait for the swap to finish in an iteration. 
% To solve this problem, we propose to perform swapping in a pipelined manner and in the background.
% Specifically, \trick\ views each model layer's swapping as one pipeline stage and pipelines kernel launching, data movement, and foreground model forwarding. For example, when layer 3 launches the swap kernel, layer 2 moves its data, and layer 1 performs normal forwarding. \yiying{Zijian, correct?}

%We launch layer $i+1$'s swapping kernel after layer $i$'s kernel launch process, which can be hidden by layer $i$'s kernel execution. The asynchronous transfer of layer $i+1$'s KV will be performed along with layer $i$'s computation and other operations that preceds the attention kernel at layer $i+1$. 
% When layer $i$ is launching CUDA data-movement kernel, layer $i+1$ performs the actual data movement as its kernel has been launched in the previous time unit, and layer $i+2$ performs normal decoding as it has finished all data movement.
% \yiying{correct, Zijian?}
%We design a swap scheme to fully overlap swap kernel launching and data movement in a layer-by-layer pipeline way.
% With pipelining, we hide both the kernel launch overhead and data movement.
%, allowing us to treat swapping as ``free'' as long as we do not exceed the swap limit, $N_i$, as described below.
%swap in and swap out are serially executed

\boldunderpara{Swap chunking.}~~~
Another major bottleneck with the primitive \swap\ is that it swaps out (in) all the context of a request at the iteration when an API is called (returns), delaying the iteration and causing memory waste from other running requests. 
%With limited swap bandwidth, the time to finish swapping out could be much higher than what the iteration would normally take (on decoding and prefill). The longer iteration time not only delays the starting of the next iteration and impacts request completion time but also wastes the GPU memory occupied by other requests while waiting for the swap to finish. Similarly, when an API call finishes, swapping in the request context could take longer than a normal iteration. 
To further reduce memory waste beyond swap pipelining, 
%To mitigate this issue, we borrow the idea from chunked prefill~\cite{chunk_prefill_sarathi} 
we propose to chunk swap out and swap in across multiple iterations so that in each iteration, the swap latency can be hidden by overlapping it with model forwarding. At iteration $i$ with batch size $B_i$, we set $T_{swap}(N_i) = T_{forward}(B_i)$ and solve for $N_i$, which we call the \textit{swap limit}. This fully overlaps all swapping with model forwarding.

% \vspace{-0.1in}
% \begin{equation}
% N_i = Batch_i \times T_{forward} / S_{swap}
% \end{equation}
% \vspace{-0.1in}

% At each iteration, we only swap out and in at most $N_i$ tokens, leaving the rest to future iterations. We call $N_i$ the {\em swap limit}.
%If the total number of tokens to be swapped out or in exceeds $N_i$, we 

\boldunderpara{Determining swap-in and swap-out budget.}~~~
%determine swap limit
%Swap limit is decided by the batch size. batch size is determined by the batch formation: number of running requests plus number of waiting requests that we can add without crossing the compute saturation point or GPu memory space. compute saturation point (beyond that no improvement of throughput)
At every iteration, there can be tokens waiting to be swapped out and swapped in.
\trick\ determines how much bandwidth to give to swap out and to swap in at each iteration
%from the swap limit ($N_i$) at each iteration. 
%We make this decision 
by maximizing inference throughput (\ie, the number of tokens that can be added to an iteration's processing) while guaranteeing the following criteria:
1) the total swap in and out amount of tokens should be at most $N_i$;
2) the amount of swapped-out memory should not exceed the amount of free CPU memory plus the swapped-in memory;
and 3) the amount of swapped-in memory and memory for newly scheduled tokens (\ie, our maximizing target) should not exceed the amount of swapped-out memory and free GPU memory. We will use the obtained swap-in and swap-out budget when deciding per-request preemption schedule in \S\ref{sec:inter-request}.

%After solving the above linear equation, we know the swap-in and swap-out budget (in terms of number of tokens). Yet, we still need to decide what requests to use the swap-in budget and the swap-out budget if there are more requests waiting for swap in/out than the limit. We leave the discussion of this decision to \S\ref{sec:inter-request}.

%swap out vs swap in split of bandwdith: solve linear equation at static time by
%maximizing swap in tokens + scheduled batch tokens, while ensuring:
%1. swap in tokens + scheduled tokens <= swap out tokens + free GPU memory
%2. swap in time + swap out time <= iteration time (iteration time profiled)
%3. swap out amount - swap in amount <= free CPU memory
%assuming at each iteration there are always plenty tokens to swap in and to swap out 

\subsection{Recomputation Chunking}
\label{sec:improve-discard}

%\boldunderpara{Recomputation chunking.}~~~
%The naive implementation of \improvediscard\ performs recomputation of an API-returned request in the iteration that the request is next scheduled for. (\eg, $i_6$ in Figure~\ref{fig-existing}). 
With the straightforward implementation of \discard\ and \improvediscard, the entire context of an API request is set as the prompt of the resumed request. 
The recomputation of the context is thus equivalent to the prefill stage of a new request with the same prompt length, which is expected to run in one iteration with state-of-the-art inference systems~\cite{vLLM,Orca}. 
%recomputation of the entire context for an API request happens in one iteration.
%involves the model forwarding that is equivalent to the prefill of a prompt of the context length, which could consume a significant amount of GPU resources. To finish the recomputation in one iteration (default scheme for prefill), one would need to preempt other running requests to free GPU resources for the recomputation. Moreover, 
% Adding the recomputation of long context to an iteration increases the iteration time. The remaining running requests' occupied GPU resources are wasted during the extra iteration time. 
% Worse, when there are not enough GPU resources to host the context, some running requests need to be preempted to free their resources.

To fully utilize the GPU, \trick\ borrows from Sarathi ~\cite{chunk_prefill_sarathi} and chunks the recomputation of long contexts into multiple iterations. In each iteration, we chunk recomputation so as not to exceed $S$, the \textit{saturation point}. Decoding utilizes less GPU compute than recomputation (equivalent to decoding vs. prefill). As iteration batches are mostly filled with decoding requests, we can merge them with recomputation requests to saturate both GPU memory and compute. 
%(which is equivalent to recomputation). Our observation is that the recomputation of a context is equivalent to the prefill of a prompt of the same context length. Both recomputation and prefill have higher computation needs than decoding under the same memory needs. When more requests in a batch are performing decoding, then there will be more GPU computation resources (\ie, GPU core time) left for recomputation. 
% We capture the relationship between the number of decoding requests, context lengths of running requests, and $K_i$ by performing an offline regression step. We then use the captured linear equation to calculate $K_i$ at the run time. \yiying{above correct?}

%kernel used for attention computation from scratch (no kv cache available): use xformer 
%otherwise, use deepspeed kernel. for multi query, parallelize queries with flashattention.

\subsection{GPU Memory Waste Calculation}
\label{sec:memory-waste}

%While swap can happen for free with our optimized implementation and as long as we do not exceed the swap limit, discard and preserve each has its pros and cons, as discussed in \S\ref{sec:existing-study}. To decide which of them to use for a request, we need a unified metric to quantify their impacts on inference throughput. Our proposal is to measure the potential GPU memory waste, i.e. size \x time, for each strategy at a request-level. On modern server-grade GPUs like A100~\cite{XXX} and \fixme{XXX}, GPU memory is the bottleneck that limits the amount of computation supported. By quantifying the GPU memory waste incurred by each strategy, we can weigh different strategies' impact on the overall inference performance.

%First, we reason about GPU memory by assigning a decision for each paused request. This is done by computing a waste term for each decision: preserve, discard, and swap. The decision with the least waste is selected. We formulate waste as a unit of memory-time. The waste from preserving a request is straightforward: for as long as a request is blocked on its API call, it occupies memory that cannot be accessed by running requests. The waste from discarding/swapping a request comes from having to recompute/swap its context; this adds latency to the recomputation iteration, which wastes memory occupied by running requests. In essence, eviction adds pure time to an iteration which instead could have been used to execute more iterations of the running group.

\boldunderpara{Memory waste of preserve.}~~~
The waste from preserving a request is straightforward: for as long as a request is blocked on its API call, it occupies GPU memory that cannot be accessed by running requests. Thus, the preserve waste $P_{j}$ for request $j$ is the API execution time, $T_{API}$, multiplied by the amount of GPU memory held by the request's context, $C_j$.

\begin{equation}
P_j = T_{API} \times C_j
\end{equation}

% $S$ is a constant that can be determined offline according to LLM model size. %\trick\ finds $C_i$ simply by examining the number of tokens seen by a request. 
The memory held by a request's context is the number of tokens in the sequence multiplied by the per-token memory usage. The per-token memory is model-specific and is obtained from the model architecture specification.
Determining $T_{API}$ is less straightforward. From \S\ref{sec:study}, we find some API types with fairly stable execution time that can be profiled offline. For these API types, we simply use the offline profile of the corresponding type to set $T_{API}$. Other API types can have huge variations in their execution times. Moreover, there can be API types not profiled offline. For both cases, we use an algorithm to be described in \S\ref{sec:unknown-api}. 

\boldunderpara{Memory waste of discard.}~~~
Discarding a request's context at API calling time immediately frees its GPU memory. However, it incurs GPU memory waste when recomputing the context for the request to resume from the API call. This waste comes from two aspects.
First, the recomputing itself consumes memory that is not useful for producing any new tokens.
As we perform recomputation in a chunked fashion (\S\ref{sec:improve-discard}), at each iteration, we are adding a chunk of memory waste that lasts until all recomputation finishes. To simplify the calculation, we assume a consistent number of sequences at the normal decoding stage in each iteration. Then we use the allowed batch size at the iteration when API is called, $K$, as the recomputation chunk size when it's resumed. To fully recompute a context length of $C$, we thus need $\frac{C}{K}$ iterations.
Then the total memory waste to perform recomputation is $ (K+ 2K + 3K + ... + nK) \times T_{forward}(S)$ where $n = \frac{C}{K}$.

Apart from the above waste, another waste caused by recomputation is due to the added iteration time. %As discussed in \S\ref{sec:improve-discard} 
Specifically, \trick charges recomputation with slowing down the generation speed of other normal sequences. This can be translated into our waste measurement with the equation: $T_{added} \times S_{run}$, where $T_{added}$ is the amount of iteration time that is attributed to the recomputation chunk in that batch and $S_{run}$ stands for the GPU memory occupied by other sequences. Similarly, we use the system state at the API call time to estimate the resume time.

% recomputating a long context can increase iteration time even with chunking. We find that the execution time of an iteration can be expressed as a linear function of the number of tokens in the batch. With the offline profiler, we obtain this linear function $f(num-tokens)$. During the run time, we use this function to find the iteration time with and without recomputation tokens, which is the added iteration time because of recomputation, \ie, $f(S_{run}+S_{recomp}) - f(S_{run})$.
%to capture the relationship between the running group size ($f(S_{run}$), the recomputation size ($f(S_{recomp}$), and the added iteration time because of the recomputation. \yiying{fill what exact this equation is？ or something about the quality of the fitting} 
% During this added time, the memory occupied by the non-API running requests is wasted, and this amount is $(f(S_{run}+S_{recomp}) - f(S_{run})) \times S_{run} \times S $.

%To obtain the recomputation waste, we profile the model and hardware to model the relationship between the number of query tokens in a batch and the corresponding model forwarding time. We denote this term as $f(x)$ where $x$ is the number of tokens in the batch. The unique latency added by recomputation is $f(c)$, and the memory wasted during this time is the sum of all memory utilized by the running group $R$. Additionally, we resume a request in chunks to maximize decoding throughput. The chunk size $c_h$ is $B - |R|$ where $B$ is the number of batch tokens required to meet the throughput saturation point and $|R|$ is the size of the running group. It will take $n = \lceil c / c_h \rceil$ iterations to resume the request in its entirety, which means the chunks that are resumed earlier are wasted. This waste is the following: $(c_h + 2c_h + ... + nc_h) * f(c_h) = (1 + 2 + ... + n) * c_h * f(c_h) = \frac{(n + n^2)}{2} * c_h * f(c_h)$.

Adding these two parts, we have the total recomputation memory waste $D_i$ as 

% \begin{equation}
% D_i = (f(S_{run}+S_{recomp}) - f(S_{run})) \times S_{run} \times S + \frac{n \times (n+1)}{2} \times T_i 
% \end{equation}
\begin{equation}
D_i = T_{added} \times S_{run} + \frac{n \times (n+1)}{2} \times T_i \times S_{K}
\end{equation}

\if 0
\boldunderpara{Memory waste of swap.}

Finally, we also profile the per-token swapping latency, and denote this as $s(x)$ where $x$ is the number of tokens that are swapped. Since memory needs to be both swapped in and out, this term is multiplied by 2.
\begin{equation}
swap_i = 2 * s(c_i) * \sum^R_r c_r
\end{equation}

While we do not know the true size of the running group, we observe that the amount of memory consumed by the running group stabilizes once the system is in a steady state. 
Once each of these terms is computed for all paused requests, we select $\textbf{argmin}_i \{preserve_i, discard_i, swap_i\}$ for each request.
\fi

\subsection{Inter-Request Action Decision}
\label{sec:inter-request}

\S\ref{sec:improve-swap}, \S\ref{sec:improve-discard}, and \S\ref{sec:memory-waste} lays the building blocks for making the scheduling decision for API calling time and resume time. We now discuss how the \trick\ scheduler makes the final decision by considering multiple requests together.

We refer to each request that is blocked on an API call as a \textit{paused} request.
In iteration $i$ for a paused request $j$, we set its memory waste $W_{ij} = \textbf{min} (P_{ij}, D_{ij})$. This is the decision for each request that the scheduler will follow.
Next, we sort  all requests making API calls in descending order of their memory waste. 
We then swap out paused requests until we run out of swap-out budget.
% For example, suppose the swap-out budget is 2000 tokens, and the highest-waste request's context is 1000, the second highest's being 500, and third highest's being 800.
% The first two requests' context can be completely swapped out, with the third one still leaving 300 tokens and all the remainin requests' context tokens to handle.
Finally, we preserve or discard based on the decision determined by the waste equation.
%With the waste calculation of discard and preserve for each request and the 
%first decide preserve or not preserve, based on whether memory spent on preserving context is higher or lower than memory wasted because recomputation overhead

%Then for the not preserve requests, rank them by recomputation memory waste.

%Then we swap from the highest discard waste request as much as we can (until the swap limit). if swap limit not hit, go to the next highest disacrd waste request. and so on.

When a discarded or swapped request is \textit{resumed} (its API finishes), we add the request to the waiting queue and ensure it is ordered by their original arrival times to the system (first come first serve).
% The waiting queue contains all requests ready to be served, including newly arrived requests that have never been served before, API requests that have been discarded and returned from API calls, and API requests that have been swapped out and returned.
We schedule the waiting queue purely based on resource availability, namely GPU memory. Once a request is scheduled, we chunk its recomputation (and/or chunk its swap-in) up to the saturation point (and/or swap-in budget). We greedily fill these limits to maximize inference throughput.

% At the beginning of each iteration, we check if there is room to add waiting requests without exceeding the GPU resource limit. If so, we choose the waiting request that arrives the earliest. If the request has tokens swapped out, we swap in tokens as much as the swap-in budget allows. If the free room (in terms of the number of tokens) is not enough to cover the chosen waiting request, we leave the remaining tokens of the request in the waiting queue for processing in the next iteration(s). If there is more free room after the first waiting request, we go to the next request in FCFS order until free room runs out.
%at each iteration, swap in as much as the swap limit allows. swap requests based on FCFS (request arrival rate). 
%Apart from the decision of swapping in, we also need to decide at each iteration what 
%To decide between requests in the waiting queue (either new or previously discarded) and requests that can be swapped in (previously swapped), we use FCFS.


%\subsection{Iterative Batch Formation}
%\label{sec:batch-form}

%how many waiting requests to add

%what waiting requests to choose

\input{fig-e2e-lat}
\input{fig-e2e-tput}
\subsection{Dealing with Unknown API Time}
\label{sec:unknown-api}

For some APIs, the execution time may be unknown or difficult to estimate, even with a profile. Without knowing the API execution time,  we cannot properly determine the preserve waste, $P_i$, using Equation\ref{XXX}, which in turn affects the decision of whether to preserve or discard an API request. To accommodate unknown API execution time, we implement an LRU (least recently-used) policy that computes $\hat{T}_{API} = t_{now} - t_{call}$ where $t_{now}$ is the current timestamp and $t_{call}$ is the timestamp at which the API was invoked. This has the effect of penalizing APIs the longer they stay in the system and preserving shorter APIs, avoiding hasty discarding.

% use a decaying method that keeps updating the waste calculation in the following way. 
% Initially, we assign the request a short, constant API time, $T_{init}$.
% After $T_{init}$ has passed, if the API has not finished yet, we increase the API time by $d$, \ie, to $T_1 = d \times T_{init}$. We follow this pattern and increase the API time by $d$ times when the previously set API time has passed. 
% We empirically set $T_{init}$ and $d$ by performing an offline profiling step. 
%When the API execution time is unknown, we use a short initial prediction. Then, we decay the prediction each time it is exceeded. We compare various initial predictions and decay rates to an oracle on an A6000 machine on the mixed dataset. We hide the API execution time of all requests from the system.






















\if 0
%In this work, we build an LLM serving system, Vulcan, that supports extensive augmented LLM models and develop a new scheduler that addresses the issues outlined in \S~\ref{sec:study}. The high-level overview of Vulcan is depicted in \fixme{xxx}. Vulcan implements preemptive scheduling for sequences making API calls, i.e. paused requests, and employs a novel algorithm to estimate the cost/benefit of preemption. Specifically, we propose to use \textit{GPU resource waste}, which stands for unused GPU memory over a certain amount of time, as the estimation criteria. In each forwarding iteration, our scheduler selects a subset of paused sequences as the preemption targets according to the estimated waste, then passively preempts them as needed.

%In the following sections, we first articulate the scheduling algorithm in \S~\ref{sec:alg}. Then we describe our optimized preemption mechanism that jointly considers evicting and discarding KV caches of paused sequences in \S~\ref{sec:fpreempt}.

\boldunderpara{API execution time.}
1) The longer an API executes, the more memory*time we can potentially reuse. => We should favor discarding tokens from longer-running APIs like chatbot over short-running ones like calculator, so as to increase the ratio of <memory (size*time) saved>/<recomputation needed>
2) API calls have different execution times. Some API types like calculator have predictable (stable) execution time, while others are unpredictable (\eg, when a user responded in a chatbot). => For predictable API times, we can give priority to short ones when choosing requests to discard/swap blocks. For unpredictable API times or for adjusting for wrong predictions, we need a dynamic way to adapt the priority of a request in terms of block discarding and swapping.
3) For predictable API time requests, we can explore the possibility of pre-recomputing of earlier tokens just in time before the API returns.

maintain three request queues: running, paused (API calls being made or normal requests intercepted), and waiting (new requests waiting to start).
For each request, we track its context length and the number of tokens being cached in kv cache.

two types of memory blocks: active (those currently being used by running requests) and inactive (not currently used). For inactive blocks, we first group them by their corresponding requests' API call remaining time. Then, within each group, we sort blocks by their positions in the corresponding sequence (from earliest to latest).

When an API call is triggered, we add its context (current cached KVs) to the corresponding inactive block group based on the API type. Here, we assume that we can estimate the API call time based on the call type and input to the call, we will discuss how we deal with unknown API call times in \S\ref{sec:unknown-api}. 
We round robin requests within the longest-running API group for K rounds by swapping out earliest tokens. Then round robin the second longest-running API group for K rounds, etc. If we run out of blocks from API groups, we need to swap/discard regular blocks from non-API running requests, and we add these blocks to the inactive block group with API time zero, \ie, the bottom group.

When an API returns or when there is room for a paused non-API request, we need to swap in or recompute discarded tokens of it plus computing the API returned tokens (for API requests). \fixme{mechanism for recomputation to be filled.}

% \input{fig-transformer-block}

\boldunderpara{Getting $f(x)$}
To accurately determine the iteration time, the first question to answer is: what independent variables can control the workload of a full model forwarding pass? From our profiling results, we find that linear layers and attention layers account for nearly \emph{95\%} of the total execution time of the transformer block. Thus we only study the behaviour of these operations in this work.

The linear layers apply matrix multiplication to all input tokens, meaning its computation complexity scales linearly to the batch size. If a batch contains one request processing its prompt tokens, all tokens from that sequence will be forwarded in that iteration, which results in a large batch size that can easily saturate the GPU utilization. In this case, the mapping between the batch size and the layer execution time would be highly accurate. However, this is not always true, as the number of inflight tokens can be arbitrarily small because of the limited GPU memory capacity. For example, if all requests in a batch are performing normal decoding, the device memory would have to hold the KV value for all history contexts to generate a new token. This small batch size leads to memory-bounded computation if not fully occupying streaming multiprocessors, which adds complexity to our mapping function to describe this behavior. Existing works such as \fixme{add deepspeed and chunk-prefill paper} propose to fuse prompt stage sequences with normal decoding ones in each iteration to stabilize the number of inflight tokens. We also adopt this technique to maintain a reasonably large batch size across iterations so that our function only needs to cater to more predictable scenarios. More details about our chunking policy can be found in Sec\fixme{add text for our prefill-chunk, include profile, conservative scheduling to prevent looking far into future. }

Additionally, we study the performance of self-attention kernel, which takes QKV matrices of input sequences and computes the attention score for each query. This kernel can contribute more than \emph{50\%} of the overall forwarding time when most of the sequences in a batch are in the normal decoding phase. Thus, it is equally important for our estimation function to capture its behavior when predicting the model runtime. In attention operation, each sequence will calculate its attention score separately but concurrently. The computation complexity and the amount of memory access can depend on the number of queries and sequence length for each sequence, which creates a group of tasks with ragged workloads competing for GPU resources. Instead of mapping from the fine-grained batch composition to the kernel performance, we find that the execution time of the attention kernel stays consistent if the running workload requires the same amount of device memory, which is always the case in a production environment where the GPU memory is fully occupied by the KV cache. \fixme{add arithmetic plot for arith intensity} This finding aligns with the fact that attention calculation is heavily memory-bounded because of its low arithmetic intensity. This also remains true even with the adoption of FlashAttention implementation.

Combining these two insights, we choose to build our iteration time predictor around a single factor: the total number of inflight tokens in the batch. We perform offline profiling on the given GPU hardware and fit a linear model that maps the batch size to the model forwarding time.

%We first need to decide how many tokens to recompute/compute within each iteration, based on batch size to achieve good throughput for the mixed decoding-recomputation iteration, while controling request latency. Then, for each iteration, we check if there's enough GPU memory. If not, we trigger the discard algorithm above.

\fi


==> fig-discard.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/discard.pdf}}
%\vspace{-0.1in}
\mycaption{fig-discard}{Illustration of Default, Improved, and \sys\ Discard.}
{
Vertial: GPU resources occupied or wasted by API and other requests.
Horizontal: timeline divided by iterations (dotted vertical lines). %API call is triggered at the end of 2nd iteration and finishes at the end of the 5th iteration.
Hatch parts represent memory waste.
}
\end{center}
%\vspace{-0.1in}
\end{figure}
}


==> fig-e2e-lat.tex <==
{
\begin{figure*}[t]
\begin{center}
\centerline{\includegraphics[width=0.95\textwidth]{Figures/e2e_mixed_lat.pdf}}
\vspace{-0.05in}
\mycaption{fig-e2e-lat}{Normalized Latency against Request Arrival Rate.} 
{
Lower right is better, \ie, sustains higher serving load.
}
\end{center}
%\vspace{0.2in}
\end{figure*}
}


==> fig-e2e-tput.tex <==
{
\begin{figure*}[t]
\begin{center}
\centerline{\includegraphics[width=0.95\textwidth]{Figures/e2e_mixed_tput.pdf}}
\vspace{-0.05in}
\mycaption{fig-e2e-tput}{Throughput against Request Arrival Rate }
{
Throughput expressed as completed requests per second. Higher is better.
}
\end{center}
% \vspace{0.3in}
\end{figure*}
}


==> fig-e2e-ttft.tex <==
{
\begin{figure*}[t]
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Figures/e2e_mixed_ttft.pdf}}
%\vspace{-0.1in}
\mycaption{fig-e2e-ttft}{Time-to-first-token (TTFT) with 6B and 13B models on the mixed workload}
{
}
\end{center}
%\vspace{-0.1in}
\end{figure*}
}


==> fig-preserve.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{Figures/preserve.pdf}}
%\vspace{-0.1in}
\mycaption{fig-swap}{Illustration of \preserve.}
{
%Vertial: GPU resources occupied or wasted by API and other requests.
%Horizontal: timeline divided by iterations (dotted vertical lines). %API call is triggered at the end of 2nd iteration and finishes at the end of the 5th iteration.
%Hatch parts represent memory waste.
}
\end{center}
%\vspace{-0.1in}
\end{figure}
}


==> fig-swap.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/swap.pdf}}
%\vspace{-0.1in}
\mycaption{fig-swap}{Illustration of Default and \sys\ Swap.}
{
%Vertial: GPU resources occupied or wasted by API and other requests.
%Horizontal: timeline divided by iterations (dotted vertical lines). %API call is triggered at the end of 2nd iteration and finishes at the end of the 5th iteration.
%Hatch parts represent memory waste.
}
\end{center}
%\vspace{-0.1in}
\end{figure}
}


==> fig-transformer-block.tex <==
%\begin{figure}[!htb]
%\centering
%\includegraphics[width=\columnwidth]{Figures/api_props_2x2/short_workload.pdf}
% \vspace{-15pt}
%\caption{The workloads Alfword, Gkmls, and HotpotQA all represent short workloads. The Alfworld incrementally explores a virtual environemnt, causing a variable high number of calls. The Alfworld also has a very large initial context length due to a description of the environment in a ReAct fashion. In terms of return length, the HotPot dataset has a higher context length, representing the retrieval length.}
%\label{fig:cdf_api_properties_short}
% \vspace{-15pt}
%\end{figure}
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/block_arch.png}}
%\vspace{-0.1in}
\mycaption{fig-transformer-block}{Architecture overview of a decoding block}
{
We mainly focus on predicting the performance of attention layers (in green) and linear layers (in purple).
}
\end{center}
%\vspace{-0.1in}
\end{figure}
}



==> impl.tex <==
\input{fig-arch}

\section{Implementation: \sys}
\label{sec:impl}

%\subsection{\sys\ Overview}
%\label{sec:overview}

We implement \trick\ on top of vLLM and build {\em \sys}, an inference system designed for API-augmented LLMs. As shown in Figure~\ref{fig-arch}, \sys\ includes an API executor that performs different API calls, an iterative-level scheduler that forms a batch of waiting requests and (partial) paused requests, a swap manager that facilitates GPU/CPU memory swapping, a running status monitor that monitors the resource usage and size of running requests, a waste estimator that calculates GPU memory waste for each API-paused request, and an offline profiler that collects basic systems metrics before starting serving.

At the end of each iteration, the scheduler gathers all requests that trigger API calls, adds them to the paused-request queue, swaps as much context (computed keys and values) of paused requests as allowed to CPU memory, determines whether to preserve or discard the remaining context of each paused request based on the GPU memory waste amount calculated by the waste estimator, and calls the actual API. When an API call finishes, \sys\ determines how many swapped-out or discarded tokens to swap in or recompute in the next iteration. It also determines how many waiting requests (non-API paused requests) to schedule in the next iteration. When all the context of a paused request has been restored, \sys\ adds the tokens returned by the API call to the resumed request.



==> intro.tex <==
\section{Introduction}
\label{sec:intro}


Large language models (LLMs)~\cite{GPT4,touvron2023llama} have shown immense potential in various applications, including natural language understanding and content generation. %With the ability to capture the content in vast amounts of text data and generate coherent, contextually relevant responses, LLMs have become an essential tool for automation and information retrieval in many people's real lives.
Nonetheless, LLMs alone can only handle language-related tasks. To extend LLMs' capabilities to diverse tasks, a recent trend is to augment LLMs with other tools~\cite{parisi2022talm,schick2023toolformer,hao2023toolkengpt,the-llm-api-survey-paper} such as arithmetic calculation~\cite{hao2023toolkengpt}, information retrieval~\cite{yao2022react}, image generation~\cite{XXX}, virtual-environment interaction~\cite{shridhar2020alfworld}, text-to-speech generation~\cite{XXX}, and many other plugins~\cite{chatgpt-plugin}. 
Another type of augmented LLM extends the capabilities of a single execution of an LLM by building a longer conversation, such as chatbots~\cite{XXX} and chain-of-thoughts~\cite{XXX}.
%Augmented large language models, often accessed through APIs or integrated into applications like chatbots and plugins, extend the capabilities of LLMs to a wide range of tasks and platforms. 
We can view the use of tools and the interaction with humans or the outside world all as LLMs {\em calling APIs}. %An API call can be the invocation of a calculator, the initiation of a web retrieval, or waiting for a human to input the next command/question in a chatbot. %In API-augmented LLM environments, an LLM usually determines the type of API call, the parameter to the call, and when a call should be made based on its generated text, while the execution of the API is separated from the LLM.
% Probably a good place to mention OpenAi Plugibns, Toolbench, ToolkenGPT. 
% Describing context with excellent tool-use capabilities of state-of-the-art (SOTA) closed-source LLMs, e.g., ChatGPT

APIs have unique properties that bring new problems to LLM inference systems:
{\bf P1)} When an API call is made, the normal decoding phase is pre-empted and can only resume when the API call returns.
{\bf P2)} The context length (\ie, already computed sequence) when an API call is triggered varies from request to request and cannot be known deterministically. 
It is unclear how to deal with contexts when an API is being called.
{\bf P3)} An API's execution time varies drastically across API types and sometimes even for the same API type. For example, a calculator API finishes in less than 1\,ms, while it can take a human one minute to digest and type a subsequent chat prompt. Varying API execution time further complicates context management and request scheduling.
%web retrieval APIs often take tens of seconds. One human interacting with a chatbot can type the next chat within a few seconds, while another human may take minutes to do so. 
%P4) API call returns multiple tokens, all of which need to be processed before further decoding can happen, and the number of tokens being returned is non-deterministic. 

%From API property P1,  Two key issues to solve are what to do with already computed context (\ie, keys and values of prompt tokens and already generated tokens) at the preemption (\ie, API calling) time and how to resume a preempted request when an API call returns. 

%None of today’s LLM inference systems~\cite{vLLM,Orca} are designed for API-augmented LLMs. 
Although many LLM inference systems have been proposed in the past few years~\cite{vLLM,Orca,li2023alpaserve,aminabadi2022deepspeed,nvidia2023fastertransformer,chunk_prefill_sarathi}, none target API support.
Without the capability of handling APIs, the only way to use them for API-augmented LLMs is to treat the API preemption as the end of a request and to use a shim layer outside the inference system for handling API calls. The inference system would return a request to the shim layer when an API call is generated and treat the request as completed. The shim layer triggers and waits for the API call. Upon API return, the shim layer forms a new request with all prompt and generated tokens plus the API-returned tokens and sends the new request to the inference system. Without knowing anything about previous computations, the inference system would perform the prefilling step of the new request's prompt, causing the {\em recomputation} of all previously processed tokens' keys and values. This recomputation wastes GPU resources that other requests could have otherwise used. 

As the default API approach described above involves unnecessary recomputation(we call it \discard), a seemingly feasible approach 
%We call this approach {\em }, as it discards all computed context at API calling time. %The \discard\ scheme frees up memory occupied by API requests, which could be immediately used by other running or waiting requests. However, it could 
%\discard\ involves significant recomputation
%To avoid recomputation, a simple approach 
to extend existing LLM inference systems is to preserve a request's context (\ie, keys and values of already processed tokens) during an API call and to resume the request with the preserved context when the API call returns; we call this approach {\em \preserve}. \preserve\ avoids recomputation altogether, but the preserved context occupies GPU memory for the entire API call time. Unlike \discard, the preserved memory cannot be used for other requests' computation, which in turn hurts the overall throughput. 

To avoid recomputation and memory preserving, another possible approach to extend LLM inference system is to swap contexts to CPU memory when an API is called (we call it {\em \swap}). Although \swap\ avoids recomputation and GPU memory wastage, the limited GPU-CPU memory swapping speed could slow down the whole system.

\textit{How should an LLM inference system efficiently support API calls?}

To answer this question, we first gain deep knowledge of API natures by running LLMs augmented with a set of typical APIs, including arithmetic, question-and-answer, virtual environment, chatbot, image generation, and text-to-speech transformation.
We measure their API call execution time, frequency of making API calls, API call returned sequence length, and context lengths when an API call is made. Overall, we find that APIs exhibit bimodal execution time, with some types always finishing within 1 second and others finishing in tens of seconds to minutes. Moreover, context and API return lengths vary across API types. 

We then evaluate how well the state-of-the-art LLM inference system, vLLM~\cite{vLLM}, and the two possible extensions (\preserve\ and \swap) perform with APIs. Being API agnostic, vLLM spends more than 80\% of its time on recomputing already seen tokens. On the other hand, \preserve\ leaves nearly half of GPU memory unused for more than 60\% of the time because of API calls. Finally, \swap\ can add more than 20\% overhead to each inference iteration's time. These issues of \discard, \preserve, \swap\ lead to lower inference throughput, longer request completion time, and delayed time to first token generation.

%The second contribution of this paper is the evaluation of API-augmented LLMs on existing LLM inference systems and a comparison of \discard\ and \preserve.
%We evaluated two LLM models: GPT-J~\cite{GPT-J}, which has 6B parameters, and Baichuan~\cite{baichuan}, which has 13B parameters.
%\fixme{explain why we chose these two models}

Based on our findings, we build \sys, the {\em first} inference system targeting API-augmented LLMs. 
\sys\ adaptively chooses the strategy for handling context memory within and across requests: when a request calls an API, its memory blocks can be preserved in GPU, discarded, and/or swapped to CPU memory. Deciding among these three strategies for each request is challenging, as they have different tradeoffs. Our idea is to map all tradeoffs to a quantifiable value: the amount of GPU {\em memory wastage}. For preserve, the memory waste comes from unused context memory; for discard, it is the memory used for recomputation; for swap, it is the memory occupied by the entire batch waiting for the swap to finish.

On top of the per-request memory waste calculation, we propose algorithms to choose discard/swap blocks across requests, to handle APIs with unpredictable execution time, to determine the bandwidth given to swapping in vs. swapping out, and to dynamically decide the amount of waiting requests to add to a batch at every iteration.

%we propose an adaptive swap-based approach where we swap a dynamically chosen set of computed keys and values to CPU memory for requests making API calls. 
Finally, we propose mechanisms to hide swapping performance overhead by overlapping swapping with normal decoding and use a kernel that parallelize the attention computation of multiple API returned tokens.
%Doing so avoids the recomputation performance overhead in \discard\ and the memory waste in \preserve.

%With this approach, we build \sys, the {\em first} inference system targeting LLM APIs. 
We implement \sys\ on top of vLLM~\cite{vLLM}. We evaluate \sys, vLLM, \preserve, and \swap\ on an A100 GPU using two LLM models (GPT-J-6B~\cite{GPT-J} and Vicuña-13B~\cite{vicuna2023}) and the six API types we study.
Overall, \sys\ sustains 1.6\x{} higher serving load compared to vLLM while maintaining similar latency per token generation. \sys\ also achieves over 2\x{} completed requests per second and improves time to first token by up to 34\x{}.
%, all while maintaining the similar latency and improving .
%\fixme{Summarize results}


%At the end of each iteration, \sys\ decides how many attention keys and values to swap out to CPU memory based on the memory needs from awaiting requests and the CPU-GPU bus bandwidth. \sys\ decides what keys and values to swap out by prioritizing requests with longer API execution times. We further propose a self-adaptive way to handle APIs with unpredictable execution times. In the next iteration, we immediately give the swapped-out memory space to waiting requests. On the completion of an API, \sys\ swaps in its swapped-out memory from CPU to GPU. Finally, we observe that CPU memory space can run out, in which case we fall back to \discard.


\if 0
We make several observations and insights from these unique API properties.
First, an API call should not be treated as the end of the current request and the start of a new request, as contexts have already been computed for the tokens generated before the API call. A naive solution and what today's inference systems support is discarding all such contexts and treating all tokens when an API call returns as a new request to essentially recompute their attention scores. A request with APIs should also not be treated as a normal non-API request that continuously performs autoregressive decoding. A non-API request would have all its context in memory (at least up until when GPU memory is saturated), but keeping all context in memory for APIs would significantly waste GPU memory, as an API can pause a request for arbitrarily long. \yiying{(may also talk about swap here, depends on the swap results)}

Implication of 2): Different API calls have different implications on the decision of where their computed context memory blocks (called ``blocks'' hereafter) should remain. Intuitively, a longer-running API's context should be discarded and recomputed upon the API's return, and a short-running one's context should be preserved in GPU or swapped to CPU. However, \fixme{TODO, talk about how this decision is not easy to make and what it could potentially depend on}

Implication of 3): Different from normal decoding that decodes one token at a time, we need to process all API returned tokens (plus discarded tokens) when an API returns. How and when we process these tokens can affect not only this request's end-to-end latency but also the whole system's throughput.

As none of these simple schemes alone could work well for API-augmented LLM inference, we need to answer a series of research questions to find the best scheme to perform LLM inference with API calls. {\bf Q1}) When an API is called in a request, {\em how many tokens shall we preserve, discard, and swap}? {\bf Q2}) {\em What tokens} within a request should be preserved, discarded, or swapped? {\bf Q3}) What is the best way of {\em performing swapping and recomputation} (discarding)? {\bf Q4}) How do we make the decisions of Q1 and Q2 {\em across different requests}? {\bf Q5}) {\em What factors} affect the answer to Q1, and how to tolerate {\em non-deterministic factors}? 

This paper answers these questions and presents the {\em first} inference system targeting LLM APIs, {\em \sys}. %, by answering the key research question of \textit{how to handle context blocks for API calls}. 

Based on our GPU environment characterization and insights on LLM inferencing, we propose mechanisms to optimize the performance of swapping and recomputation (Q3). 
For swapping, our finding is that 

For recomputing discarded tokens, we propose \yiying{Reyna fill the actual algo and talk about benefits}

Based on our API workload study, we find that API execution time and context lengths are the two key factors for determining Q1.

Based on our study results, we propose several ideas in \sys. First, we propose an adaptive algorithm for choosing preserve, swap, or discard memory blocks. For unknown API time, we propose a multi-level-queue-based algorithm. \yiying{Once Vikranth has the algo, fill this part}

Our answer to Q4 is a partial request strategy. Instead of always discarding, swapping, or preserving a whole sequence, we discard (same number of?) blocks from requests within a group, and we choose to discard from the front of the sequences. \yiying{todo: talk about the benefits, Reyna can fill more and improve this part} 
%\hyperlink{https://docs.google.com/presentation/d/1zcbKbDkiGqa0uFebLausRz0QW-irAaPGo_J5MG3B3tQ/edit?usp=sharing}{slides}


\fixme{Eval results}

This paper makes the following contributions:

\begin{itemize}

\item A comprehensive study of LLM APIs and accompanying API-based LLM datasets.

\item \sys, an inference system designed for LLM API support.

\item Insights about various tradeoffs for handling LLM contexts, which could be used beyond the API setting.

\end{itemize}
We will make \sys\ publicly available upon the acceptance of the paper.
\fi


\if 0
1. what to do with already computed kvs when an API call is made


2. what request to run when an API call is being made
=> FCFS or other scheduling policy?

3. how to process API returned tokens
=> kernel to use and number of thread blocks to use

4. when to process API returned tokens
=> chunk vs not chunk (affects overall throughput and tail latency)

%5. how to perform beam search

why not use huge CPU memory (like TBs of big servers)

up to \fixme{XXX}\x\ times
\fi

==> references.tex <==
\pagestyle{empty}

\bibliographystyle{}
\bibliography{references}

==> related.tex <==
\section{Related Works}
\label{sec:related}


==> tbl-free-swap.tex <==
\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{ |c|c|c|c|}
\hline
  Workload & Context Len & 2 A6000 & 8 A100 \\
 \hline
{GPT-j-6B, total swap} & 1024 & 972 & 337 \\
{GPT-j-6B, for resume} & 1024 & 422 & 104 \\
\hline
{baichuan-13B, total swap} & 1024 & 545 & nan \\
{baichuan-13B, for resume} & 1024 & 208 & nan \\
% {GPT-j-6B, swap in} & 731 & 209/2 \\
 \hline
\end{tabular}
\mycaption{tbl-free-swap}{``Free'' swap tokens.}
{
\textbf{Total swap} means the number of tokens that can be swapped out/in without affecting foreground performance. \textbf{For resume} means the number of tokens that can be resumed with swap after fulfilling the current batch's added memory requirement with swapping. The batch composition follows chunk-prefill style wherein a chunk of size \textit{free recompute} is bin-packed with normal decoding.
}
\end{center}
\end{table}


==> tbl-unknown-api.tex <==
\begin{table}
\centering
\captionsetup{justification=centering, singlelinecheck=false, font={it,small}}
\caption{Unknown API Time}
\begin{tabular}{c|ccccc}
\hline
\textbf{$T_{init}$} & \textbf{0.5s} & \textbf{1s} & \textbf{5s} & \textbf{10s} & \textbf{LRU} \\
\hline
\% of Oracle & 92.79 & 96.99 & 93.19 & 76.99 & 93.19 \\
\hline
\end{tabular}
\label{tab:unknown}
\end{table}

